Ages and Metallicities of Early-Type Void Galaxies from Line Strength Measurements

We present spectroscopic observations of 26 galaxies of type E and S0, based on their blue morphologies, located in voids by the study of Grogin & Geller (1999). Measurements of redshift, velocity dispersion, and four Lick line indices, Mgb, Fe5270, Fe5335, and Hbeta with their errors are given for all of these galaxies, along with Hbeta, [OIII], Halpha, and [NII] emission line strengths for a subset of these objects. These sources are brighter than M star for low density regions and tend to be bluer than their counterpart early-type objects in high density regions. Using the models of Thomas et al. (2003) gives metal abundances and ages with a median alpha enhancement, [alpha/Fe] = +0.13, and median metals abundance, [Z/H] = +0.22, values comparable to those found for E and S0 galaxies in clusters, but with a wider spread in [Z/H] towards low values. If the emission line subsample is interpreted as younger, the proportion of young objects is higher than for early-types in higher density regions. There is a significant incidence of sources in the sample with emission lines in their spectra (46% with Hbeta and [OIII] and 69% with Halpha or [NII]) as well as shells and rings in their morphologies (19%). The diagnostic log[NII/Halpha], log[OIII/Hbeta] diagram places 10 of 12 emission line galaxies in or near the star forming and liner region and two among the Seyferts. The Halpha fluxes indicate star formation rates of 0.2 to 1.0 Msun per yr. The percentage of these early-type void galaxies undergoing star formation appears to be higher compared to their cluster counterparts and the range of ages wider.

==> tab1.tex <==
1 & 15R 464.015505 & 00 03 36.098 & +10 36 12.54 &  8085 & S0 &-19.00 &-20.50  & -23.84\\
2 & CGCG 0027.9+0536 & 00 30 28.637 & +05 51 39.06 &  7238 & E2 &-19.15 &-20.59  & -24.03\\
3 & NGC 476 & 01 20 19.952 & +16 01 12.40 &  6439 & S0 &-18.78 &-20.37 & -23.81\\
4 & IC 1700 & 01 25 24.652 & +14 51 52.43 &  6484 & E0(shells) &-20.12 &-21.64 & -25.01\\
5 & CGCG 0133.6+1734 & 01 36 20.281 & +17 48 58.01 &  6065 & E2 &-18.10 &-19.71  &-23.11 \\
6 & CGCG 1348.4+3517 & 13 50 38.973 & +35 02 18.09 &  6407 & E0 &-19.55 &-21.01  & -24.42\\ 
7 & CGCG 1429.5+3929 & 14 31 27.815 & +39 15 32.14 &  7038 & SB0 &-19.22 &-20.73 & -24.15\\
8 & CGCG 1433.0+2311 & 14 35 17.143 & +22 57 46.34 &  6336 & SB0(ring)&-18.54 &-19.84 & -23.06\\
9 & CGCG 1434.7+4010 & 14 36 42.686 & +39 56 37.64 &  6217 & E1 &-18.72 &-20.19 & -23.74\\
10 & CGCG 1506.2+2208 & 15 08 29.040 & +21 56 51.73 &  6259 & S0 &-18.82 & -20.42& -23.72\\
11 & 15R 328.038850 & 15 33 41.477 & +28 08 44.24 &  5772 & S0/a & -16.95&-18.35  & -21.73\\
12 & CGCG 1536.8+3707 & 15 38 38.464 & +36 57 30.18 &  5751 & S0 &-19.02&-20.37  &-23.76\\
13 & CGCG 1549.1+2551 & 15 51 13.249 & +25 42 05.11 &  6546 & S0 &-19.33 &-20.85  & -24.18\\
14 & CGCG 1552.1+3018 & 15 54 11.455 & +30 09 21.35 &  6175 & E0 &-18.30 &-19.82 & -23.39\\
15 & CGCG 1600.6+4302 & 16 02 16.663 & +42 54 59.66 &  7541 & S0(ring) &-19.77 & -20.98 & -24.21\\
16 & CGCG 1607.5+4152 & 16 09 16.555 & +41 44 43.47 &  7891 & S0 &-19.37 &-20.81 & -24.15\\
17 & CGCG 2108.7+0318 & 21 11 15.074 & +03 31 19.42 &  5342 & E3 &-18.17 & -19.51 & -22.79\\
18 & NGC 7113 & 21 42 26.650 & +12 34 07.35 &  5989 & S0 &-19.20 & -20.89& -24.59\\
19 & CGCG 2140.0+1340 & 21 42 26.896 & +13 53 58.61 &  5631 & E2 & -18.58& -20.22 &-23.63 \\
20 & 15R 518.119354 & 21 50 27.756 & +12 38 08.91 &  6850 & S0/a &-17.27 & -18.82  & -22.29\\
21 & 15R 520.029201 & 22 35 05.336 & +10 55 25.89 &  5240 & E0 &-16.76 &-18.05  & -21.50\\
22 & CGCG 2236.9+1336 & 22 39 21.911 & +13 52 54.19 &  5423 & S0(ring) &-17.93 & -18.66&-20.89 \\
23 & NGC 7509 & 23 12 21.430 & +14 36 33.41 &  5118 & E0+star &-19.36 & -21.01 & -24.37\\
24 & NGC 7550 & 23 15 16.007 & +18 57 42.49 &  5340 & E0 &-20.29 &-21.98  & -25.45\\
25 & 15R 523.044360 & 23 37 38.094 & +12 06 00.42 & 8104 &  S0(shells)&-18.00 & -18.92 &-21.74 \\
26 &15R 523.036286 & 23 44 29.634 & +11 40 48.01 & 7090 & SB0    & -18.98 & -20.38 & -23.09\\


==> tab4.tex <==
01&  10.2&  0.5&  0.19&  0.09&  0.14&  0.08\\
 02& 10.1&  0.2&  0.01&  0.06&  0.11&  0.07\\
 03&  9.8&  0.3&  0.04&  0.04&  0.07&  0.04\\
 04&  9.6&  0.2&  0.31&  0.08&  0.09&  0.08\\
 05&  9.7&  0.2&  0.17&  0.05&  0.06&  0.08\\
 06&  9.9&  0.3&  0.24&  0.09&  0.10&  0.09\\
 07& 10.0&  0.3&  0.44&  0.09&  0.19&  0.10\\
 08&  9.9&  0.3& -0.27&  0.07&  0.23&  0.14\\
 09&  9.3&  0.3&  0.39&  0.18&  0.12&  0.13\\
10&  9.9&  0.3&  0.44&  0.10&  0.18&  0.10\\
11&  9.6&  0.3& -0.65&  0.27&  0.24&  0.34\\
12&  10.2& 0.5& -0.12&  0.04&  0.08&  0.06\\
13&  9.6&  0.3&  0.45&  0.07&  0.13&  0.09\\
14& 10.0&  0.3&  0.22&  0.04&  0.36&  0.06\\
15&  9.0&  0.5&  0.26&  0.04&  0.12&  0.05\\
16&  9.8&  0.2&  0.33&  0.08&  0.13&  0.09\\
17&  9.3&  0.2& -0.15&  0.05&  0.09&  0.08\\
18&  9.7&  0.3&  0.24&  0.08&  0.30&  0.06\\
19&  9.9&  0.3&  0.18&  0.03&  0.17&  0.04\\
20&  9.8&  0.3& -0.12&  0.09&  0.18&  0.14\\
21&  \gg15&   - &     -&     -&     -&     -\\
22&  3$<$&     -&     -&     -&     -&     -\\
23& 10.2&  0.3&  0.22&  0.04&  0.30&  0.06\\
24&  9.6&  0.3&  0.53&  0.07&  0.04&  0.07\\
25&  3$<$&     -&     -&     -&     -&     -\\
26&  \gg15&   - &     -&     -&     -&     -\\

